Goupil: A Monte Carlo engine for the backward transport of low-energy gamma-rays

Goupil is a software library designed for the Monte Carlo transport of low-energy gamma-rays, such as those emitted from radioactive isotopes. The library is distributed as a Python module. It implements a dedicated backward sampling algorithm that is highly effective for geometries where the source size largely exceeds the detector size. When used in conjunction with a conventional Monte Carlo engine (i.e., Geant), the response of a scintillation detector to gamma-active radio-isotopes scattered over the environment is accurately simulated (to the nearest percent) while achieving events rates of a few kHz (with a ~2.3 GHz CPU).

==> table-rocks.tex <==
\begin{tabular}{ll}
\toprule
    Mineral  & Fraction ($\%$) \\
\midrule
    SiO2  & 50.7 \\
    Al2O3 & 16.4 \\
    FeO   & 11.0 \\
    MgO   &  4.7 \\
    CaO   & 10.5 \\
    Na2O  &  2.9 \\
    K2O   &  1.1 \\
    TiO2  &  1.0 \\
    MnO   &  0.2 \\
    P2O5  &  0.2 \\
    H2O   &  1.3 \\
\bottomrule
\end{tabular}

